Optimized Multi-Token Joint Decoding with Auxiliary Model for LLM Inference

Large language models (LLMs) have achieved remarkable success across diverse tasks, yet their inference processes are hindered by substantial time and energy demands due to single-token generation at each decoding step. While previous methods such as speculative decoding mitigate these inefficiencies by producing multiple tokens per step, each token is still generated by its single-token distribution, thereby enhancing speed without improving effectiveness. In contrast, our work simultaneously enhances inference speed and improves the output effectiveness. We consider multi-token joint decoding (MTJD), which generates multiple tokens from their joint distribution at each iteration, theoretically reducing perplexity and enhancing task performance. However, MTJD suffers from the high cost of sampling from the joint distribution of multiple tokens. Inspired by speculative decoding, we introduce multi-token assisted decoding (MTAD), a novel framework designed to accelerate MTJD. MTAD leverages a smaller auxiliary model to approximate the joint distribution of a larger model, incorporating a verification mechanism that not only ensures the accuracy of this approximation, but also improves the decoding efficiency over conventional speculative decoding. Theoretically, we demonstrate that MTAD closely approximates exact MTJD with bounded error. Empirical evaluations using Llama-2 and OPT models ranging from 13B to 70B parameters across various tasks reveal that MTAD reduces perplexity by 21.2% and improves downstream performance compared to standard single-token sampling. Furthermore, MTAD achieves a 1.42x speed-up and consumes 1.54x less energy than conventional speculative decoding methods. These results highlight MTAD's ability to make multi-token joint decoding both effective and efficient, promoting more sustainable and high-performance deployment of LLMs.

==> sections/methodology_RWBSD.tex <==

\section{Methodology}

\subsection{Beam Speculative Decoding}

%Introduce beam speculative decoding. The drawback is low accepted length.
A straightforward idea to achieve better efficiency and effectiveness over greedy decoding is to fuse beam decoding and speculative decoding. A possible way is to use the small model to generate a draft beam sampling tree, and use the target model to verify each layer of the tree by considering the joint beam sampling probability of all the nodes in that layer. By utilizing the idea of rejection sampling and speculative decoding, it is possible to guarantee each layer has the identical sampling distribution as beam sampling. However, since all the nodes at the same layer are accepted/rejected together, it is possible that a whole layer is rejected because of only one node with bad quality. As a result, the average acceptance rate will be low and the decoding efficiency will be compromised. 

To alleviate the problem, we first introduce a relaxed version of beam decoding, named random width beam decoding, which relaxes the fixed beam width $M$ to a random variable with range $[M_1,M_2]$. We empirically show than RWBD still has better sampling effectiveness than greedy decoding.
Then we introduce \fullname{}, which accelerates RWBD with the idea of speculative decoding while achieves the identical sampling distribution.  Since the beam width of RWBD is flexible, \method{} can accept/reject each node at the layer independently, which leads to better acceptance rate and thus better decoding efficiency.

\begin{definition}
    \textit{\textbf{Random Width Beam Decoding (RWBD)}}. Let $M_1,M_2$ denote the minimum and maximum number of beam width for RWBD. At each sampling step, given $m^\prime$ ($M_1\le m^\prime\le M_2$) input sequences, RWBD samples $m$ output sequences based on the joint likelihood where $m\in[M_1,M_2]$ is a random integer. 
\end{definition}

We can see that beam decoding is a special case of RWBD where $M_1=M2$, and greedy decoding is a special case where $M_1=M_2=1$.

Intuitively, the effectiveness of RWBD is determined by $\mathbb{E}(m)$. We provide empirical evidences to support our assumption. 
Specifically, ...
Therefore, $\mathbb{E}(m)>1$, RWBD should be more effective than greedy decoding.

Now, we introduce random width speculative beam decoding, which accelerates random width beam decoding with the asssitance of a small draft model.

\begin{figure}
    \centering
    \includegraphics[width=0.98\linewidth]{figures/VerifySample.pdf}
    \caption{Illustration of how \method{} verify the beam sampling tree.}
    \label{fig:verifysample}
\end{figure}

\textbf{Overview.} 
Let $M_1,M_2$ be the minimum and maximum beam width, and let $\gamma$ be the maximum number of tokens generated at each iteration. 
% Small model generates beam sampling tree
\method{} first exploits a small model to generate a beam sampling tree with beam width $M_2$ and depth $\gamma$.
% Large model computes the next token probability for all the nodes in the tree, which can be used to compute the sampling probability of beam sampling with the target model.
Then the target model takes the sequences represented by all the tree nodes as inputs and computes the next-token distribution for each node. These next-token distributions are later used to compute the sampling distribution of beam sampling with the target model.
% Verify  
After that, \method{} verifies each layer of the beam search tree sequentially. At each layer, it accepts the nodes that \emph{can} lead to an identical distribution to RWBD. If a node is rejected, then all its children are rejected. If the number of accepted nodes is larger than minimum beam width, then \method{} continues to verify the next layer. Otherwise, the verification terminates.
% sample
When verification terminates, it is either because a layer is rejected or it reaches the last layer. And an additional layer is sampled with $M_2$ output sequences based on either the adjusted residual distribution or the beam sampling distribution of the large model.

\textbf{Details of Sampling Iteration}
Let $\mathcal{T}$ denote the beam sampling tree, $\mathcal{T}_i$ denote the $i$-th layer of $\mathcal{T}$, and $\mathcal{T}_{i,j}$ denote the $j$-th node at $i$-th layer. Let $\bm{s}_{ij}$ denote the sequence represented by node $\mathcal{T}_{ij}$. Let $\bm{b}_i\in\mathbb{R}^{M_2}$ denote the beam score vector at layer $i$, which represents the joint likelihoods of input sequences at each beam sampling step. At the beginning of the verification, we have $\bm{b}_1=\bm{1}$. 
% Details of computing joint likelihood, not right
When verify the $i$-th ($i=1,\ldots,\gamma$) layer, \method{} first computes the beam sampling distribution: 
\begin{equation}
P_{beam}(\bm{s}|LM_L,\mathcal{T}_{i-1})\propto\left\{\begin{aligned}
    &\bm{b}_{i}[k]P_{token}(\bm{s}[-1]|LM_L,prefix,\bm{s}[:-1]),\quad &\bm{s}[:-1]\in\mathcal{T}_{i-1}\\
    &0,\quad &\bm{s}[:-1]\notin\mathcal{T}_{i-1}
\end{aligned}
\right.
\end{equation}
where $\bm{s}[-1]$ is the last token in $\bm{s}$, $\bm{s}[:-1]$ is the subsequence of $\bm{s}$ before the last token, $k$ is the index of $\bm{s}[:-1]$ in $\mathcal{T}_{i-1}$ and $\bm{b}_i[k]$ is its beam score.

% Details of verification
After that, \method{} verifies each sequence $\bm{s}_{ij}$, $j=1,\ldots,M_2$ sequentially. Figure \ref{fig:verifysample} gives an example illustration of the verification. First, let $p=P_{beam}(\bm{s}|LM_L,\mathcal{T}_{i-1})$ and we accept $\bm{s}_{i1}$ with probability $1-\frac{p(\bm{s}_{i1})}{P_{beam}(\bm{s}_{i1}|LM_S,\mathcal{T}_{i-1})}$ where $P_{beam}(\bm{s}|LM_S,\mathcal{T}_{i-1})$ is the beam sampling probability of the small model. If $\bm{s}_{i1}$ is rejected, the distribution $p$ is adjusted to the residual distribution, i.e., $p=norm(\max(0,p-P_{beam}(\bm{s}|LM_S,\mathcal{T}_{i-1})))$ where $norm$ denotes the normalization operation. Then we verify $\bm{s}_{i2}$ with the adjusted $p$. If for some $j$ $\bm{s}_{ij}$ is accepted, then $p$ is reset to $P_{beam}(\bm{s}|LM_L,\mathcal{T}_{i-1})$. 
For all rejected sequences, their beam score is set to 0, which forces the sampling probability of its children to be 0. For all accepted sequences $\bm{s}_{ij}$, their beam score is set to $P_{beam}(\bm{s}_{ij}|LM_L,\mathcal{T}_{i-1})$. 
After verifying all the nodes at layer $i$, if there are less than $M_1$ sequences accepted, then the verification terminates and all the unverified layers are discarded. Otherwise, \method{} keeps verifying the next layer.
Let layer $l$ be the last accepted layer. After verification, \method{} generates an additional layer by sampling $M_2$ sequences $s_{l+1,1},\ldots,s_{l+1,M_2}$ from $P_{beam}(\bm{s}|LM_L,\mathcal{T}_l)$. The sequences $s_{l+1,1},\ldots,s_{l+1,M_2}$ are the input of the next \method{} sampling iteration.

The pseudocode of \method{} is illustrated in Algorithm \ref{alg:method}.

\begin{algorithm}
\caption{\textsc{\fullname{}}}
\label{alg:method}
\begin{algorithmic}[1]
\Require $LM_S,LM_L,prefix,M_1,M_2,\gamma$
\Ensure output sequence $output$
\State $input\leftarrow prefix$
\While{true}
\State $input\leftarrow$ \textsc{\method{}Step}($input,LM_S,LM_L,M1,M2,\gamma$)
\If {\textsc{StopCriterion}($input$) = true}
\State \textbf{break}
\EndIf
\EndWhile
\State $output\leftarrow$ best sequence in $input$
\State \Return $output$
\State 
\Procedure{\textsc{\method{}Step}}{$input,LM_S,LM_L,M_1,M_2,\gamma$}
  \State $\mathcal{T}\leftarrow$ \textsc{BeamSample}($input,LM_S,M_2,\gamma$) 
  \State //\texttt{$\mathcal{T}[i,j]$ is the $j$-th output sequence at step $i$}.
  \State $\mathcal{P}\leftarrow$ \textsc{GetNextTokenProb}($LM_L,\mathcal{T}$)
  \State //\texttt{Use target model to compute next-token distribution for $\gamma M_2$ sequences in $\mathcal{T}$.}
  \State $BeamScore\leftarrow \bm{1}$
  \For{$i=1,\ldots,\gamma$}
  \State $\mathcal{S}\leftarrow\mathcal{T}[i]$
  \State $\mathcal{V}, terminate, BeamScore \leftarrow$\textsc{Verify}($\mathcal{P},\mathcal{S},BeamScore,M_1,M_2$)
  \If{$terminate = true$}
  \State \Return $\mathcal{V}$
  \EndIf
  \EndFor
  \State // \texttt{all steps accepted, sample next step}
  \State $P_{beam}(\bm{s}|LM_L)\leftarrow BeamScore*P_{token}(s_{-1}|LM_L,\bm{s}_{:-1})/\sum_{}BeamScore$
  \State \Return $\{s_j|s_j\sim P_{beam}(\bm{s}|LM_L), j=1,\ldots,M_2\}$
\EndProcedure
\State
\Procedure{\textsc{Verify}}{$\mathcal{P},\mathcal{S},BeamScore, M_1,M_2$}
\State $P_{beam}(\bm{s}|LM_L)\leftarrow BeamScore*P_{token}(s_{-1}|LM_L,\bm{s}_{:-1})/\sum_{}BeamScore$
\State $p(\bm{s})\leftarrow P_{beam}(\bm{s}|LM_L)$
\State $cnt\leftarrow 0$
\State $\mathcal{V}\leftarrow \emptyset$
\For{$\bm{s}_j\in \mathcal{S}$}
\State $\tau\sim U(0,1)$
\If{$\tau\le p(\bm{s}_j)/P_{beam}(\bm{s}_j|LM_S)$}
\State //\texttt{draft sequence passes verification}
\State $\mathcal{V}.append(\bm{s}_j)$
\State $BeamScore(\bm{s}_j)\leftarrow P_{beam}(\bm{s}_j|LM_L)$, $p(\bm{s})\leftarrow P_{beam}(\bm{s}|LM_L)$, $cnt\leftarrow cnt + 1$
\Else 
\State // \texttt{set beam score to 0 to mark rejection}
\State $BeamScore(\bm{s}_j)\leftarrow 0$ 
\State // \texttt{update $p$ to residual distribution}
\State $p(\bm{s})\leftarrow norm(\max(0,p(\bm{s})-P_{beam}(\bm{s}|LM_S)))$
\EndIf
\EndFor
\If{$cnt < M_1$}
\State //\texttt{Sample more sequences}
\While{$cnt < M_2$}
\State $\bm{s}\sim p(\bm{s})$, $\mathcal{V}.append(\bm{s})$, $cnt\leftarrow cnt+1$, $p(\bm{s})\leftarrow P_{beam}(\bm{s}|LM_L)$
\EndWhile
\State $terminate\leftarrow true$
\Else
\State $terminate\leftarrow false$
\EndIf
\State \Return $\mathcal{V}, terminate, BeamScore$
\EndProcedure
\end{algorithmic}    
\end{algorithm}


\begin{theorem}\label{theorem:exact}
    Let $\mathcal{I}=\{input_1,\ldots,input_{m^\prime}\}$ be the input sequences to a sampling step of the random width beam sampling, where $M_1\le m^\prime \le M_2$. Let $P(\bm{s}|LM_L,\mathcal{I})$ denote the probability that the output sequence $\bm{s}$ is sampled by the target model $LM_L$ based on the inputs $\mathcal{I}$. Let $\bm{s}_1,\ldots,\bm{s}_m$ be the output sequence generated by our proposed speculative sampling step (see Algorithm ?), where $m\in\{1,\ldots,M_2\}$ is an implicit random variable determined by how many draft sequences are accepted. We have 
    \begin{equation}
        \bm{s}_i\stackrel{\text{i.i.d.}}{\sim}P(\bm{s}|LM_L,\mathcal{I}),\quad i=1,\ldots,m
    \end{equation}
\end{theorem}

The proof is given in the Appendix.
